A Rooted Structure Theorem for $5$-Connected Graphs and $K_6^-$-Minors

Jorgensen conjectured that every $6$-connected graph with no $K_6$-minor is apex. For a $6$-connected graph containing a $K_4$ on vertices $a_1,\dots,a_4$, being apex is equivalent to $G-a_i$ having a planar embedding with the other three roots on a common face for some $i$, so that for such graphs the conjecture becomes a rooted planarity statement. Robertson, Seymour, and Thomas showed that the failure of the corresponding three-rooted planarity is witnessed by a legless tripod. We introduce a four-root structure, called a frame, that extends this certificate, and prove a structural theorem: every $5$-connected graph containing a frame rooted at four prescribed vertices contains a subgraph of one of five explicit types, denoted $A$--$E$. This theorem does not depend on the edges among the roots. As an application, we show that when the four roots span a $K_4^-$, each of the five configurations yields a $K_6^-$-minor. Together with a planar argument for the case without a frame and an induction based on a theorem of Kawarabayashi, this gives a proof that every non-planar $5$-connected graph contains a $K_6^-$-minor. This statement also follows from a recent theorem of Lo; our proof is independent and is driven by the rooted structure theorem, whose method we expect to apply to Jorgensen's conjecture with other target configurations.

==> figures/S1toS2_graph.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v1) at ($(sp)!0.75!(a4)$);
    \coordinate (v2) at ($(sp)!0.75!(a3)$);
    \coordinate (v3) at ($(sp)!0.5!(a3)$);
    \coordinate (v4) at ($(s)!0.5!(a2)$);



    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setBHL] (s)--(a1);
    \draw[setBHL] (s)--(sp);
    \draw[setBHL] (v1) to[bend right=18](v2);
    \draw[setBHL] (v1)--(a4);
    \draw[setBHL] (sp) -- (a3);
    \draw[setBHL] (v3) to[bend right=18] (v4);
    \draw[setBHL] (v4) -- (a2);

    

    \draw[setAHL] (t)--(a1);
    \draw[setAHL] (t)--(a2);
    \draw[setAHL] (t)--(a3);

    \draw[setCHL] (sp)--(v1);





    

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);
    \draw[Spath] (s)--(sp);



    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v1) to[bend right=18] (v2);

    

    \draw[Hpath] (v3) to[bend right=18] (v4);




    #1

    \foreach \p in {s,sp,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,sp,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {v1,v2,v3,v4}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, above=2pt] at (sp) {$s_2$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, right=2pt] at (v1) {$v_1$};
    \node[redPlainLbl, left=2pt] at (v2) {$v_2$};
    \node[redPlainLbl, right=2pt] at (v3) {$v_3$};
    \node[redPlainLbl, left=2pt] at (v4) {$v_4$};




\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/S1toS3.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v1) at ($(s)!0.8!(a1)$);
    \coordinate (v2) at ($(t)!0.5!(a1)$);
    \coordinate (v3) at ($(s)!0.55!(a1)$);
    \coordinate (v4) at ($(s)!0.55!(a3)$);


    \coordinate (vs) at ($(t)!0.5!(a2)$);

    \coordinate (b4) at ($(s)!0.3!(a1)$);
    \coordinate (b4r) at ($(s)+(1.10,1.15)$);
    \coordinate (b4l) at ($(s)+(-0.80,1.15)$);
    \coordinate (b4d) at ($(b4)+(-0.55,0.85)$);
    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setAHL] (b4)--(a1);
    \draw[setAHL] (v3) to[bend left=18](v4);
    \draw[setAHL] (v4)--(a3);

    

    \draw[setBHL] (t)--(a1);
    \draw[setBHL] (t)--(a2);
    \draw[setBHL] (t)--(a3);
    \draw[setBHL] (s)--(a4);
    \draw[setBHL] (s) to [bend left=18](vs);


    \draw[setAHL, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);

    \draw[setCHL] (s)--(v4);
    \draw[setCHL] (v1) to [bend left=18] (v2);

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v3) to[bend left=18] (v4);
    \draw[Hpath] (s) to[bend left=18] (vs);
    \draw[Hpath] (v1) to[bend left=18] (v2);

    

    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);




    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {b4,v1,v2,v3,v4,vs}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=4pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};
    \node[redPlainLbl, left=2pt] at (v1) {$v_3$};
    \node[redPlainLbl, right=2pt] at (v2) {$v_4$};
    \node[redPlainLbl, left=2pt] at (v3) {$v_1$};
    \node[redPlainLbl, right=2pt] at (v4) {$v_2$};
    \node[redPlainLbl, right=2pt] at (vs) {$v_0$};



\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/S1toS3n2.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v1) at ($(s)!0.8!(a1)$);
    \coordinate (v2) at ($(t)!0.5!(a1)$);
    \coordinate (v3) at ($(s)!0.55!(a1)$);
    \coordinate (v4) at ($(s)!0.55!(a3)$);

    \coordinate (vs) at ($(t)!0.5!(a2)$);

    \coordinate (b4) at ($(s)!0.3!(a1)$);
    \coordinate (b4r) at ($(s)+(1.10,1.15)$);
    \coordinate (b4l) at ($(s)+(-0.80,1.15)$);
    \coordinate (b4d) at ($(b4)+(-0.55,0.85)$);
    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setDHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \path[name path=svs] (s) to[bend left=18] (vs);
    \path[name path=vthreevfour] (v3) to[bend left=18] (v4);
    \path[name intersections={of=svs and vthreevfour, by=v5}];

    \draw[setAHL] (s)--(a2);
    \draw[setAHL] (s)--(a3);
    \draw[setAHL] (s)--(a4);

    

    \draw[setBHL] (b4)--(a1);
    \draw[setBHL] (t)--(a2);
    \draw[setBHL] (v2)--(t);
    



    \draw[setBHL, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);

    \draw[setCHL] (s)--(b4);
    \draw[setCHL, intersection segments={of=svs and vthreevfour, sequence=L1}];
    \draw[setCHL, intersection segments={of=svs and vthreevfour, sequence=R1}];
    \draw[setDHL, intersection segments={of=svs and vthreevfour, sequence=L2}];
    \draw[setDHL, intersection segments={of=svs and vthreevfour, sequence=R2}];
   
    \draw[setBHL] (v1) to [bend left=18] (v2);

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v3) to[bend left=18] (v4);
    \draw[Hpath] (s) to[bend left=18] (vs);
    \draw[Hpath] (v1) to[bend left=18] (v2);

    

    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);




    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {b4,v1,v2,v3,v4,v5,vs}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=4pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};
    \node[redPlainLbl, left=2pt] at (v1) {$v_3$};
    \node[redPlainLbl, right=2pt] at (v2) {$v_4$};
    \node[redPlainLbl, left=2pt] at (v3) {$v_1$};
    \node[redPlainLbl, right=2pt] at (v4) {$v_2$};
    \node[redPlainLbl, below left=2pt] at (v5) {$u$};
    \node[redPlainLbl, right=2pt] at (vs) {$v_0$};



\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/S1toT3n2.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v1) at ($(s)!0.8!(a1)$);
    \coordinate (v2) at ($(t)!0.5!(a1)$);
    \coordinate (v3) at ($(s)!0.55!(a1)$);
    \coordinate (v4) at ($(t)!0.55!(a3)$);


    \coordinate (vs) at ($(t)!0.7!(a3)$);

    \coordinate (b4) at ($(s)!0.3!(a1)$);
    \coordinate (b4r) at ($(s)+(1.10,1.15)$);
    \coordinate (b4l) at ($(s)+(-0.80,1.15)$);
    \coordinate (b4d) at ($(b4)+(-0.55,0.85)$);
    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setDHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap = round, line join = round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setBHL] (b4)--(a1);
    \draw[setDHL] (v3) to[bend left=18](v4);
    \draw[setDHL] (s)--(b4);

    


  
    \draw[setCHL] (t)--(a3);
    \draw[setAHL] (s)--(a4);
    \draw[setDHL] (s) to [bend left=4](vs);


    \draw[setBHL, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);

    \draw[setAHL] (s)--(a3);
    \draw[setAHL] (s)--(a2);

    \draw[setBHL] (v2)--(t);
    \draw[setBHL] (t)--(a2);
    \draw[setBHL] (v1) to [bend left=12] (v2);

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v3) to[bend left=18] (v4);
    \draw[Hpath] (s) to[bend left=4] (vs);
    \draw[Hpath] (v1) to[bend left=12] (v2);

    

    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);




    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {b4,v1,v2,v3,v4,vs}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, left=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};
    \node[redPlainLbl, left=2pt] at (v1) {$v_3$};
    \node[redPlainLbl, right=2pt] at (v2) {$v_4$};
    \node[redPlainLbl, left=2pt] at (v3) {$v_1$};
    \node[redPlainLbl, right=2pt] at (v4) {$v_2$};
    \node[redPlainLbl, right=2pt] at (vs) {$v_0$};



\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/S4toS3T1T2T3_graph.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);

    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v2) at ($(t)!0.44!(a3)$);
    \coordinate (v1) at ($(s)!0.74!(a4)$);


    \coordinate (b4) at ($(s)!0.5!(a1)$);
    \coordinate (b4r) at ($(s)+(1.10,1.15)$);
    \coordinate (b4l) at ($(s)+(-0.80,1.15)$);
    \coordinate (b4d) at ($(b4)+(-0.55,0.85)$);
    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setAHL] (a1)--(t);
    \draw[setAHL] (a2)--(t);
    \draw[setAHL] (a3)--(t);
    \draw[setAHL] (v1) to[bend left=36] (v2);
    \draw[setAHL] (v1)--(a4);


    \draw[setBHL] (s)--(a1);
    \draw[setBHL] (s)--(a2);
    \draw[setBHL] (s)--(a3);
    \draw[setBHL, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);
    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);

    \draw[Hpath] (v1) to[bend left=36] (v2);


    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s}
        \fill[black] (\p) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);
    \fill[red!70!black] (v1) circle (0.09);
    \fill[red!70!black] (v2) circle (0.09);
    \fill[red!70!black] (b4) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};


    \node[redPlainLbl, left=2pt] at (v2) {$v_2$};
    \node[redPlainLbl, right=2pt] at (v1) {$v_1$};

    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};



\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/S4toS3T1T2T3_graphn2.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v2) at ($(s)!0.74!(a3)$);
    \coordinate (v1) at ($(s)!0.74!(a4)$);


    \coordinate (b4) at ($(s)!0.5!(a1)$);
    \coordinate (b4r) at ($(s)+(1.10,1.15)$);
    \coordinate (b4l) at ($(s)+(-0.80,1.15)$);
    \coordinate (b4d) at ($(b4)+(-0.55,0.85)$);
    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setAHL] (a1)--(t);
    \draw[setAHL] (a2)--(t);
    \draw[setAHL] (a3)--(t);
    \draw[setCHL] (v1) to[bend right=18] (v2);
    \draw[setCHL] (v1)--(a4);


    \draw[setBHL] (s)--(a1);
    \draw[setBHL] (s)--(a2);
    \draw[setBHL] (s)--(a3);
    \draw[setBHL, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);
    
    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);

    \draw[Hpath] (v1) to[bend right=18] (v2);


    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s}
        \fill[black] (\p) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);
    \fill[red!70!black] (v1) circle (0.09);
    \fill[red!70!black] (v2) circle (0.09);
    \fill[red!70!black] (b4) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};


    \node[redPlainLbl, left=2pt] at (v2) {$v_2$};
    \node[redPlainLbl, right=2pt] at (v1) {$v_1$};

    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};



\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/allSi.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v5) at ($(s)!0.4!(a1)$);
 
    \coordinate (v3) at ($(s)!0.6!(a2)$);
    \coordinate (v4) at ($(s)!0.6!(a3)$);
    \coordinate (v1) at ($(s)!0.8!(a1)$);
    \coordinate (v2) at ($(s)!0.8!(a3)$);

    \coordinate (vs) at ($(t)!0.5!(a3)$);

    \coordinate (b4) at ($(s)!0.4!(a2)$);

    \coordinate (v3r) at ($(s)+(1,1)$);
    \coordinate (v3l) at ($(s)+(-1,1)$);
    \coordinate (v3d) at ($(v5)+(-0.55,0.75)$);



    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

  
    \draw[setAHL] (t)--(a2);
    \draw[setAHL] (t)--(a3);
    \draw[setAHL] (t)--(a1);
    \draw[setAHL] (s) to [bend right=4pt](vs);
    \draw[setAHL] (s)--(a4);

    \draw[setBHL] (v3)--(a2);
    \draw[setBHL] (v4)--(a3);
    \draw[setBHL] (v5)--(a1);
 

    \draw[setBHL,rounded corners=10pt] 
    (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (v5);

    \draw[setBHL] (v1) to [bend left=18pt] (v2);

    
    \draw[setBHL] (v3) to [bend left=18pt] (v4);

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v3) to[bend left=18] (v4);

    \draw[Hpath] (v1) to[bend left=18] (v2);


    \draw[Hpath] (s) to[bend right=4] (vs);
    
    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (v5);

    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {v1,v2,v3,v4,v5,vs}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (v1) {$v_1$};
    \node[redPlainLbl, right=2pt] at (v2) {$v_2$};
    \node[redPlainLbl, left=2pt] at (v3) {$v_6$};
    \node[redPlainLbl, right=2pt] at (v4) {$v_5$};
    \node[redPlainLbl, left=2pt] at (v5) {$b_4$};

    \node[redPlainLbl,below left =2pt] at (vs) {$v_0$};




\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/bothS3.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (b4) at ($(s)!0.5!(a1)$);
 
    \coordinate (v1) at ($(s)!0.6!(a2)$);
    \coordinate (v2) at ($(s)!0.6!(a3)$);
    \coordinate (b4p) at ($(s)!0.4!(a2)$);
    \coordinate (a) at ($(s)!0.4!(a4)$);

    
    \coordinate (v3) at ($(s)!0.8!(a1)$);
    \coordinate (v4) at ($(s)!0.8!(a3)$);


    \coordinate (vs) at ($(t)!0.4!(a1)$);

    



    \coordinate (v3r) at ($(s)+(1,1)$);
    \coordinate (v3l) at ($(s)+(-1,1)$);
    \coordinate (v3d) at ($(b4)+(-0.55,0.75)$);



    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

  
    \draw[setBHL] (t)--(a1);
    \draw[setBHL] (t)--(a2);
    \draw[setBHL] (t)--(a3);
    \draw[setBHL] (s) to [bend right=18pt] (vs);
    \draw[setBHL] (s)--(a4);


    \draw[setAHL] (b4)--(a1);
    \draw[setAHL] (v4)--(a3);

    \draw[setCHL] (v2) -- (v4);
    \draw[setCHL] (b4p) -- (v1);
    \draw[setCHL] (v1) to [bend left=18pt] (v2);

    \draw[setCHL] (b4) -- (s);




    
    

    \draw[setAHL,rounded corners=10pt] 
    (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (b4);

    \draw[setCHL] (b4p) to [bend left=18pt] (a);

    
    \draw[setAHL] (v3) to [bend left=18pt] (v4);

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v1) to[bend left=18] (v2);
    \draw[Hpath] (v3) to[bend left=18] (v4);

    \draw[Hpath] (s) to[bend right=18] (vs);



    \draw[Hpath] (b4p) to[bend left=18] (a);


    
    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (b4);

    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {b4,b4p,v1,v2,v3,v4,vs,a}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (b4p) {$b$};
    \node[redPlainLbl, right=3pt] at (a) {$a$};

    \node[redPlainLbl, left=2pt] at (v1) {$v_3$};
    \node[redPlainLbl, right=2pt] at (v2) {$v_4$};
    \node[redPlainLbl, left=2pt] at (v3) {$v_1$};
    \node[redPlainLbl, right=2pt] at (v4) {$v_2$};

    \node[redPlainLbl, left=3pt] at (b4) {$b_4$};

    \node[redPlainLbl, left=2pt] at (vs) {$v_0$};





\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/caseE.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (b4) at ($(s)!0.4!(a1)$);
 
    \coordinate (v1) at ($(s)!0.7!(a2)$);
    \coordinate (v2) at ($(s)!0.7!(a3)$);
    \coordinate (b4p) at ($(s)!0.4!(a2)$);
    \coordinate (a) at ($(s)!0.4!(a4)$);
    
    \coordinate (v3) at ($(s)!0.6!(a1)$);
    \coordinate (v4) at ($(t)!0.7!(a1)$);


    \coordinate (vs) at ($(t)!0.4!(a1)$);

    



    \coordinate (v3r) at ($(s)+(1,1)$);
    \coordinate (v3l) at ($(s)+(-1,1)$);
    \coordinate (v3d) at ($(b4)+(-0.55,0.75)$);



    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setDHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap = round, line join = round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

  
    \draw[setBHL] (t)--(a2);
    \draw[setBHL] (t)--(v4);
    \draw[setBHL] (v3) to [bend right=18pt] (v4);
    \draw[setBHL] (b4)--(a1);


    \draw[setAHL] (b4p)--(a2);
    \draw[setAHL] (a)--(a4);

    \draw[setAHL] (v2)--(a3);

    \draw[setCHL] (s) -- (a);
    \draw[setCHL] (s) -- (v2);
    \draw[setCHL] (s) to [bend right=18pt] (vs);


    \draw[setDHL] (s) -- (b4p);
    \draw[setDHL] (s) -- (b4);



    
    

    \draw[setBHL,rounded corners=10pt] 
    (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (b4);

    \draw[setAHL] (b4p) to [bend left=18pt] (a);

    
    \draw[setAHL] (v1) to [bend left=18pt] (v2);

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v1) to[bend left=18] (v2);
    \draw[Hpath] (v3) to[bend right=18] (v4);

    \draw[Hpath] (s) to[bend right=18] (vs);



    \draw[Hpath] (b4p) to[bend left=18] (a);


    
    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (b4);

    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {b4,b4p,v1,v2,v3,v4,vs,a}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (b4p) {$b$};
    \node[redPlainLbl, right=3pt] at (a) {$a$};

    \node[redPlainLbl, left=2pt] at (v1) {$v_3$};
    \node[redPlainLbl, right=2pt] at (v2) {$v_4$};
    \node[redPlainLbl, left=2pt] at (v3) {$v_1$};
    \node[redPlainLbl, left=2pt] at (v4) {$v_2$};

    \node[redPlainLbl, left=3pt] at (b4) {$b_4$};

    \node[redPlainLbl, left=2pt] at (vs) {$v_0$};





\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/crossS1T.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (b4) at ($(s)!0.3!(a1)$);
    \coordinate (v3) at ($(t)!0.65!(a1)$);
    \coordinate (v4) at ($(s)!0.4!(a2)$);
    \coordinate (v5) at ($(s)!0.6!(a1)$);
    \coordinate (v6) at ($(t)!0.2!(a1)$);


    \coordinate (v3r) at ($(s)+(1,1)$);
    \coordinate (v3l) at ($(s)+(-1,1)$);
    \coordinate (v3d) at ($(b4)+(-0.55,0.75)$);



    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

  
    \draw[setAHL] (t)--(a2);
    \draw[setAHL] (t)--(a3);
    \draw[setAHL] (v5) to [bend left=8](v6);
    \draw[setAHL] (b4)--(a1);
    \draw[setAHL] (v6)--(t);



    \draw[setBHL] (s)--(a2);
    \draw[setBHL] (v3)--(a1);
    \draw[setBHL] (s)--(a3);
    \draw[setBHL] (s)--(a4);

    \draw[setAHL,rounded corners=10pt] 
    (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (b4);


    
    \draw[setBHL] (v3) to [bend left=18pt] (v4);

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v3) to[bend left=18] (v4);

    \draw[Hpath] (v5) to[bend left=8] (v6);

    
    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (b4);

    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {b4,v3,v4,v5,v6}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};


    \node[redPlainLbl, left=2pt] at (v3) {$v_3$};
    \node[redPlainLbl, right=2pt] at (v4) {$v_4$};
    \node[redPlainLbl, left=2pt] at (v5) {$v_1$};
    \node[redPlainLbl, below left= 2pt] at (v6) {$v_2$};

    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};



\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/crossS3.tex <==
\newcommand{\typeAFrame}[3]{%
  \begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v1) at ($(sp)!0.6!(a4)$);
    \coordinate (v2) at ($(s)!0.4!(a2)$);
    \coordinate (v3) at ($(s)!0.80!(a2)$);
    \coordinate (v4) at ($(s)!0.8!(a1)$);
    \coordinate (v5) at ($(s)!0.6!(a2)$);
    \coordinate (v6) at ($(s)!0.4!(a1)$);
    \coordinate (v7) at ($(s)!0.6!(a1)$);
    \coordinate (v8) at ($(t)!0.5!(a1)$);

    \coordinate (vs) at ($(t)!0.7!(a3)$);
    \coordinate (s0) at ($(s)!0.5!(sp)$);

    \coordinate (b4) at ($(sp)!0.8!(a3)$);








    \tikzset{
      setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
      setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
      setCHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
      setDHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
      baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
      mainLbl/.style={baseLbl, text=black},
      mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
      redLbl/.style={baseLbl, text=red!70!black},
      redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
      greenLbl/.style={baseLbl, text=green!60!black}
    }


    \draw[setAHL] (v4)--(a1);
    \draw[setAHL] (v2)--(a2);
    \draw[setAHL] (v3) to [bend right=18](v4);
    \draw[setAHL] (v1) to [bend right =18] (v2);
    \draw[setAHL] (v1)--(a4);




    \draw[setBHL] (s0) to [bend right=12] (vs);

    \draw[setBHL] (t) -- (vs);
    \draw[setBHL] (t) -- (a2);
    \draw[setBHL] (s0) -- (sp);
    \draw[setBHL] (sp) -- (a3);
    \draw[setBHL] (b4) to [bend left = 18] (a4);







    \draw[setCHL] (v7) -- (v4);
    \draw[setCHL] (v8) to [bend right=18pt] (v7);
    \draw[setCHL] (v8) -- (t);

    \draw[setDHL] (s)--(v7);
    \draw[setDHL] (v5) to [bend left=18pt] (v6);
    \draw[setDHL] (s)--(v2);
    \draw[setDHL] (s)--(s0);




    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);
    \draw[Spath] (s)--(sp);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v3) to[bend right=18] (v4);

    \draw[Hpath] (v1) to[bend right=18] (v2);

    \draw[Hpath] (v5) to[bend left=18] (v6);



    \draw[Hpath] (v7) to[bend left=18] (v8);

    \draw[Hpath] (s0) to [bend right=12] (vs);

    \draw[Hpath] (a4) to [bend right=18] (b4);



    #1

    \foreach \p in {s,sp,a1,a2,a3,a4,t}
    \fill[white] (\p) circle (0.08);

    \fill[black] (s) circle (0.08);
    \fill[black] (sp) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
    \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {s0,v1,v2,v3,v4,v5,v6,v7,v8,vs,b4}
    \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, above=2pt] at (sp) {$s_2$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, right=2pt] at (v1) {$v_1$};
    \node[redPlainLbl, left=2pt] at (v2) {$v_2$};
    \node[redPlainLbl, right=2pt] at (v3) {$v_3$};
    \node[redPlainLbl, left=2pt] at (v4) {$v_4$};
    \node[redPlainLbl, right=2pt] at (v5) {$v_5$};
    \node[redPlainLbl, left=2pt] at (v6) {$v_6$};

    \node[redPlainLbl, left=2pt] at (v7) {$v_7$};
    \node[redPlainLbl, left=2pt] at (v8) {$v_8$};

    \node[redPlainLbl, right=2pt] at (vs) {$v_0$};

    \node[redPlainLbl, above=2pt] at (s0) {$s_0$};


    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};



  \end{tikzpicture}%
}

\begin{minipage}{\textwidth}
  \centering
  \typeAFrame{}{}{}
\end{minipage}


==> figures/crossed2.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v2) at ($(t)!0.4!(a2)$);
    \coordinate (v1) at ($(s)!0.7!(a2)$);

    \coordinate (vs) at ($(t)!0.5!(a3)$);



    \coordinate (b4) at ($(s)!0.4!(a2)$);

    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setBHL] (a1)--(t);
    \draw[setBHL] (a2)--(t);
    \draw[setBHL] (a3)--(t);
    \draw[setBHL] (sp)--(a4);
    \draw[setCHL] (v1) to[bend right=36] (v2);
    \draw[setBHL] (vs) to[bend left=18] (sp);



    \draw[setAHL] (b4) to[bend left=18] (a4);
    \draw[setAHL] (s)--(a1);
    \draw[setAHL] (s)--(a2);
    \draw[setCHL] (s)--(sp);

    
    \draw[Spath] (s)--(sp);
    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);


    \draw[Hpath] (v1) to[bend right=36] (v2);
    \draw[Hpath] (b4) to[bend left=18] (a4);
    \draw[Hpath] (vs) to[bend left=18] (sp);




    #1

    \foreach \p in {s,sp,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s,sp}
        \fill[black] (\p) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,sp,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);
    \fill[red!70!black] (v1) circle (0.09);
    \fill[red!70!black] (v2) circle (0.09);
    \fill[red!70!black] (b4) circle (0.09);
    \fill[red!70!black] (vs) circle (0.09);


    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, above=2pt] at (sp) {$s_2$};
    \node[mainPlainLbl, left=6pt] at (a1) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};


    \node[redPlainLbl, right=2pt] at (v2) {$v_2$};
    \node[redPlainLbl, left=2pt] at (v1) {$v_1$};
    \node[redPlainLbl, right=2pt] at (vs) {$v_0$};


    \node[redPlainLbl, left=2pt] at (b4) {$b$};



\end{tikzpicture}%
}

\typeAFrame{}{}{}

==> figures/crossed3.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v1) at ($(s)!0.8!(a2)$);
    \coordinate (v2) at ($(s)!0.8!(a1)$);

    \coordinate (v3) at ($(s)!0.4!(a2)$);
    \coordinate (v4) at ($(sp)!0.7!(a4)$);

    \coordinate (v5) at ($(s)!0.3!(sp)$);
    \coordinate (v6) at ($(t)!0.7!(a2)$);

    \coordinate (s0) at ($(s)!0.8!(sp)$);

    \coordinate (vs) at ($(t)!0.5!(a3)$);



    \coordinate (b4) at ($(s)!0.6!(a2)$);

    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setDHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setBHL] (vs)--(t);
    \draw[setBHL] (a2)--(t);
    \draw[setBHL] (sp)--(a3);
    \draw[setBHL] (sp)--(a4);
    \draw[setBHL] (s0)--(sp);
    \draw[setBHL] (vs) to[bend right=4] (s0);


    \draw[setAHL] (v1) to[bend right=36] (v2);
    \draw[setAHL] (b4) to[bend left=18] (a4);
    \draw[setAHL] (v2)--(a1);
    \draw[setAHL] (b4)--(a2);

    \draw[setDHL] (s)--(v2);
    \draw[setDHL] (s)--(v5);
    \draw[setDHL] (v5) to[bend left=36] (v6);

    \draw[setCHL] (s) -- (b4);
    \draw[setCHL] (v5) -- (s0);
    \draw[setCHL] (v3) to[bend left=36] (v4);



    
    \draw[Spath] (s)--(sp);
    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);


    \draw[Hpath] (v1) to[bend right=36] (v2);
    \draw[Hpath] (v3) to[bend left=36] (v4);
    \draw[Hpath] (v5) to[bend left=36] (v6);
    \draw[Hpath] (b4) to[bend left=18] (a4);
    \draw[Hpath] (vs) to[bend right=4] (s0);




    #1

    \foreach \p in {s,sp,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s,sp}
        \fill[black] (\p) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,sp,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);
    \fill[red!70!black] (v1) circle (0.09);
    \fill[red!70!black] (v2) circle (0.09);
    \fill[red!70!black] (b4) circle (0.09);
    \fill[red!70!black] (vs) circle (0.09);
    \fill[red!70!black] (v3) circle (0.09);
    \fill[red!70!black] (v4) circle (0.09);
    \fill[red!70!black] (v5) circle (0.09);
    \fill[red!70!black] (v6) circle (0.09);
    \fill[red!70!black] (s0) circle (0.09);



    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, above=2pt] at (sp) {$s_2$};
    \node[mainPlainLbl, left=6pt] at (a1) {$a_3$};
    \node[mainPlainLbl, left=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};


    \node[redPlainLbl, left=2pt] at (v2) {$v_2$};
    \node[redPlainLbl, right=2pt] at (v1) {$v_1$};
    \node[redPlainLbl, right=2pt] at (vs) {$v_0$};
    \node[redPlainLbl, above=2pt] at (s0) {$s_0$};


    \node[redPlainLbl, left=2pt] at (v3) {$v_3$};
    \node[redPlainLbl, right=2pt] at (v4) {$v_4$};
    \node[redPlainLbl, above=2pt] at (v5) {$v_5$};
    \node[redPlainLbl, right=2pt] at (v6) {$v_6$};



    \node[redPlainLbl, left=2pt] at (b4) {$b$};



\end{tikzpicture}%
}

\typeAFrame{}{}{}

==> figures/crossed4.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

  %  \coordinate (v1) at ($(s)!0.3!(a2)$);
  %  \coordinate (v2) at ($(sp)!0.3!(a4)$);

    \coordinate (v3) at ($(sp)!0.5!(a4)$);
    \coordinate (v4) at ($(sp)!0.5!(a3)$);

    \coordinate (v5) at ($(sp)!0.8!(a3)$);

    \coordinate (s0) at ($(s)!0.6!(sp)$);

    \coordinate (vs) at ($(t)!0.5!(a3)$);



    \coordinate (b4) at ($(s)!0.4!(a2)$);

    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setDHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setBHL] (t)--(a1);
    \draw[setBHL] (t)--(a2);
    \draw[setBHL] (t)--(a3);
    \draw[setBHL] (sp)--(a4);
    \draw[setBHL] (s0)--(sp);
    \draw[setBHL] (vs) to[bend right=4] (s0);


    \draw[setAHL] (s) -- (a1);
    \draw[setAHL] (b4) to[bend left=18] (a4);
    \draw[setAHL] (s)--(a2);
    \draw[setAHL] (b4)--(a2);

    \draw[setCHL] (s)--(s0);
    \draw[setCHL] (v5) to[bend right=36] (a1);
    \draw[setCHL] (v5) -- (sp);
  %  \draw[setCHL] (v3) to[bend right=36] (v4);



    
    \draw[Spath] (s)--(sp);
    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);


   % \draw[Hpath] (v1) to[bend left=36] (v2);
  %  \draw[Hpath] (v3) to[bend right=36] (v4);
    \draw[Hpath] (v5) to[bend right=36] (a1);
    \draw[Hpath] (b4) to[bend left=18] (a4);
    \draw[Hpath] (vs) to[bend right=4] (s0);




    #1

    \foreach \p in {s,sp,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s,sp}
        \fill[black] (\p) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,sp,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);
  %  \fill[red!70!black] (v1) circle (0.09);
  %  \fill[red!70!black] (v2) circle (0.09);
    \fill[red!70!black] (b4) circle (0.09);
    \fill[red!70!black] (vs) circle (0.09);
   % \fill[red!70!black] (v3) circle (0.09);
   % \fill[red!70!black] (v4) circle (0.09);
    \fill[red!70!black] (v5) circle (0.09);
    
    \fill[red!70!black] (s0) circle (0.09);



    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, above=2pt] at (sp) {$s_2$};
    \node[mainPlainLbl, left=6pt] at (a1) {$a_3$};
    \node[mainPlainLbl, left=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};


   % \node[redPlainLbl, left=2pt] at (v2) {$v_2$};
   % \node[redPlainLbl, right=2pt] at (v1) {$v_1$};
    \node[redPlainLbl, right=2pt] at (vs) {$v_0$};
    \node[redPlainLbl, above=2pt] at (s0) {$s_0$};


   % \node[redPlainLbl, right=2pt] at (v3) {$v_3$};
   % \node[redPlainLbl, left=2pt] at (v4) {$v_4$};
    \node[redPlainLbl, right=2pt] at (v5) {$v_1$};
    



    \node[redPlainLbl, left=2pt] at (b4) {$b$};



\end{tikzpicture}%
}

\typeAFrame{}{}{}

==> figures/crossed5.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (v1) at ($(s)!0.4!(a2)$);
    \coordinate (v2) at ($(sp)!0.3!(a4)$);

    \coordinate (v3) at ($(sp)!0.5!(a4)$);
    \coordinate (v4) at ($(sp)!0.5!(a3)$);

    \coordinate (v5) at ($(sp)!0.8!(a3)$);
    \coordinate (v6) at ($(t)!0.3!(a2)$);

    \coordinate (s0) at ($(s)!0.8!(sp)$);

    \coordinate (vs) at ($(t)!0.8!(a2)$);



    \coordinate (b4) at ($(s)!0.6!(a2)$);

    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setDHL/.style={draw=blue!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setBHL] (v6)--(a2);
    \draw[setBHL] (v4)--(a3);
    \draw[setBHL] (v3)--(a4);
    \draw[setBHL] (v3) to[bend right=36] (v4);
    \draw[setBHL] (v5) to[bend right=12] (v6);


    \draw[setAHL] (s) -- (a1);
    \draw[setAHL] (b4) to[bend left=36] (a4);
    \draw[setAHL] (s)--(a2);


    \draw[setDHL] (s)--(s0);

    \draw[setDHL] (s0) to[bend left=12] (vs);

    \draw[setCHL] (v1) to[bend left=12] (v2);
    \draw[setCHL] (sp)--(v3);
    \draw[setCHL] (s0)--(sp);
    \draw[setCHL] (sp)--(v4);
    
    \draw[Spath] (s)--(sp);
    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);


    \draw[Hpath] (v1) to[bend left=12] (v2);
    \draw[Hpath] (v3) to[bend right=36] (v4);
    \draw[Hpath] (v5) to[bend right=12] (v6);
    \draw[Hpath] (b4) to[bend left=36] (a4);
    \draw[Hpath] (vs) to[bend right=12] (s0);




    #1

    \foreach \p in {s,sp,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s,sp}
        \fill[black] (\p) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,sp,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);
    \fill[red!70!black] (v1) circle (0.09);
    \fill[red!70!black] (v2) circle (0.09);
    \fill[red!70!black] (b4) circle (0.09);
    \fill[red!70!black] (vs) circle (0.09);
    \fill[red!70!black] (v3) circle (0.09);
    \fill[red!70!black] (v4) circle (0.09);
    \fill[red!70!black] (v5) circle (0.09);
    \fill[red!70!black] (v6) circle (0.09);
    \fill[red!70!black] (s0) circle (0.09);



    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, above=2pt] at (sp) {$s_2$};
    \node[mainPlainLbl, left=6pt] at (a1) {$a_3$};
    \node[mainPlainLbl, left=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};


    \node[redPlainLbl, right=2pt] at (v2) {$v_4$};
    \node[redPlainLbl, left=2pt] at (v1) {$v_3$};
    \node[redPlainLbl, left=2pt] at (vs) {$v_0$};
    \node[redPlainLbl, above=2pt] at (s0) {$s_0$};


    \node[redPlainLbl, right=2pt] at (v3) {$v_7$};
    \node[redPlainLbl, left=2pt] at (v4) {$v_8$};
    \node[redPlainLbl, right=2pt] at (v5) {$v_5$};
    \node[redPlainLbl, left=2pt] at (v6) {$v_6$};



    \node[redPlainLbl, left=2pt] at (b4) {$b$};



\end{tikzpicture}%
}

\typeAFrame{}{}{}

==> figures/crossedS1toS2S3.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    

    \coordinate (b4) at ($(s)!0.7!(a2)$);

    \coordinate (v1) at ($(s)!0.4!(a1)$);
    \coordinate (v2) at ($(sp)!0.4!(a3)$);

    \coordinate (v0) at ($(t)!0.5!(a3)$);


    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setAHL] (a1)--(t);
    \draw[setAHL] (a2)--(t);
    \draw[setAHL] (a3)--(t);
    \draw[setAHL] (v0) to [bend left =18] (sp);
    \draw[setAHL] (sp)--(a4);



    \draw[setBHL] (s)--(a1);
    \draw[setBHL] (s)--(a2);
    \draw[setBHL] (v1) to [bend left =18] (v2);
    \draw[setBHL] (v2)--(a3);
    \draw[setBHL] (b4) to [bend left =18] (a4);


    
    \draw[Spath] (s)--(sp);
    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (b4) to [bend left =18] (a4);
    \draw[Hpath] (v1) to [bend left =18] (v2);
    \draw[Hpath] (v0) to [bend left =18] (sp);





    #1

    \foreach \p in {s,sp,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s,sp}
        \fill[black] (\p) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,sp,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \fill[red!70!black] (b4) circle (0.09);
    \fill[red!70!black] (v1) circle (0.09);
    \fill[red!70!black] (v2) circle (0.09);


    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, above=2pt] at (sp) {$s_2$};
    \node[mainPlainLbl, left=6pt] at (a1) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};

    \node[redPlainLbl, left=2pt] at (v1) {$v_2$};
    \node[redPlainLbl, right=2pt] at (v2) {$v_1$};




\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/reduced_type_b.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (0,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    \coordinate (b4) at ($(s)!0.4!(a1)$);
 
    \coordinate (v1) at ($(s)!0.6!(a2)$);
    \coordinate (v2) at ($(t)!0.5!(a2)$);
    \coordinate (b4p) at ($(s)!0.4!(a2)$);
    \coordinate (a) at ($(s)!0.4!(a4)$);



    \coordinate (v3) at ($(s)!0.6!(a1)$);
    \coordinate (v4) at ($(t)!0.5!(a1)$);


    \coordinate (vs) at ($(t)!0.5!(a1)$);


    \coordinate (v3r) at ($(s)+(1,1)$);
    \coordinate (v3l) at ($(s)+(-1,1)$);
    \coordinate (v3d) at ($(b4)+(-0.55,0.75)$);



    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

  
    \draw[setBHL] (t)--(a2);
    \draw[setBHL] (t)--(a3);
    \draw[setBHL] (t)--(a1);
    \draw[setBHL] (v3) to [bend right=18pt] (v4);
    \draw[setBHL] (b4)--(v3);
    
    \draw[setAHL] (a)--(a4);


    \draw[setAHL] (s)--(a2);
    \draw[setAHL] (s)--(a3);
    \draw[setCHL] (s) -- (b4);



    
    

    \draw[setBHL,rounded corners=10pt] 
    (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (b4);

    \draw[setAHL] (b4p) to [bend left=18pt] (a);

    
    \draw[setCHL] (v1) to [bend left=18pt] (v2);

    

    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (s)--(a3);
    \draw[Spath] (s)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath] (v1) to[bend left=18] (v2);
    \draw[Hpath] (v3) to[bend right=18] (v4);


    \draw[Hpath] (b4p) to[bend left=18] (a);


    
    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (v3r) -- (v3l) -- (v3d) -- (b4);

    #1

    \foreach \p in {s,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    
    \fill[black] (s) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \foreach \p in {b4,b4p,v1,v2,v3,v4,a}
        \fill[red!70!black] (\p) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};

    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, left=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (b4p) {$b$};
    \node[redPlainLbl, right=3pt] at (a) {$a$};

    \node[redPlainLbl, left=2pt] at (v1) {$v_3$};
    \node[redPlainLbl, left=2pt] at (v2) {$v_4$};
    \node[redPlainLbl, left=2pt] at (v3) {$v_1$};
    \node[redPlainLbl, left=2pt] at (v4) {$v_2$};

    \node[redPlainLbl, left=3pt] at (b4) {$b_4$};

    




\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/sequalssp.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-1.1,-4.4);

    

    \coordinate (b4) at ($(s)!0.5!(a1)$);
    \coordinate (b4r) at ($(sp)+(1.10,1.15)$);
    \coordinate (b4l) at ($(s)+(-0.80,1.15)$);
    \coordinate (b4d) at ($(b4)+(-0.55,0.85)$);
    
    \tikzset{
        setAHL/.style={draw=green!60!black, opacity=0.30, line width=7pt, line cap=round, line join=round},
        setBHL/.style={draw=black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        setCHL/.style={draw=red!70!black, opacity=0.24, line width=7pt, line cap=round, line join=round},
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        mainPlainLbl/.style={font=\small, text=black, inner sep=1.5pt},
        redLbl/.style={baseLbl, text=red!70!black},
        redPlainLbl/.style={font=\small, text=red!70!black, inner sep=1.5pt},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    \draw[setAHL] (a1)--(t);
    \draw[setAHL] (a2)--(t);
    \draw[setAHL] (a3)--(t);
    

    \draw[setBHL] (s)--(sp);
    \draw[setBHL] (s)--(a1);
    \draw[setBHL] (s)--(a2);
    \draw[setBHL] (sp)--(a3);
    \draw[setBHL, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);

    \draw[setCHL] (sp)--(a4);
    
    \draw[Spath] (s)--(sp);
    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);


    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(t);

    \draw[Hpath, rounded corners=10pt]
        (a4) -- ($(a4)+(0.55,0.75)$) -- (b4r) -- (b4l) -- (b4d) -- (b4);




    #1

    \foreach \p in {s,sp,a1,a2,a3,a4,t}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s,sp}
        \fill[black] (\p) circle (0.08);
    \fill[green!60!black] (t) circle (0.09);
    \foreach \p in {s,sp,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    \fill[red!70!black] (b4) circle (0.09);

    #2

    \node[mainPlainLbl, above=2pt] at (s) {$s_1$};
    \node[mainPlainLbl, above=2pt] at (sp) {$s_2$};
    \node[mainPlainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainPlainLbl, right=6pt] at (a2) {$a_2$};
    \node[mainPlainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainPlainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainPlainLbl, text=green!60!black, below=4pt] at (t) {$t$};




    \node[redPlainLbl, left=2pt] at (b4) {$b_4$};



\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}

==> figures/type_a_graph.tex <==
\newcommand{\typeAFrame}[3]{%
\begin{tikzpicture}[scale=0.73, line cap=round, line join=round]
    \coordinate (s) at (-2.15,4.4);
    \coordinate (sp) at (2.15,4.4);
    \coordinate (a1) at (-3.2,0);
    \coordinate (a2) at (-1.1,0);
    \coordinate (a3) at (1.1,0);
    \coordinate (a4) at (3.2,0);

    \coordinate (t) at (-2.15,-4.4);
    \coordinate (tp) at (2.15,-4.4);

    \draw[Spath] (s)--(sp);
    \draw[Spath] (s)--(a1);
    \draw[Spath] (s)--(a2);
    \draw[Spath] (sp)--(a3);
    \draw[Spath] (sp)--(a4);

    \draw[Tpath] (t)--(tp);
    \draw[Tpath] (a1)--(t);
    \draw[Tpath] (a2)--(t);
    \draw[Tpath] (a3)--(tp);
    \draw[Tpath] (a4)--(tp);

    \tikzset{
        baseLbl/.style={font=\small, fill=white, fill opacity=0.88, text opacity=1, inner sep=1.5pt, rounded corners=1pt},
        mainLbl/.style={baseLbl, text=black},
        redLbl/.style={baseLbl, text=red!70!black},
        greenLbl/.style={baseLbl, text=green!60!black}
    }

    #1

    \foreach \p in {a1,a2,a3,a4}
        \fill[white] (\p) circle (0.08);
    \foreach \p in {s,sp}
        \fill[black] (\p) circle (0.08);
    \foreach \p in {t,tp}
        \fill[green!60!black] (\p) circle (0.09);
    \foreach \p in {s,sp,a1,a2,a3,a4}
        \draw[black, thick] (\p) circle (0.08);

    #2

    \node[mainLbl, above=4pt] at (s) {$s_1$};
    \node[mainLbl, above=4pt] at (sp) {$s_2$};
    \node[mainLbl, left=6pt] at (a1) {$a_1$};
    \node[mainLbl, left=6pt] at (a2) {$a_2$};
    \node[mainLbl, right=6pt] at (a3) {$a_3$};
    \node[mainLbl, right=6pt] at (a4) {$a_4$};
    \node[mainLbl, text=green!60!black, below=4pt] at (t) {$t_1$};
    \node[mainLbl, text=green!60!black, below=4pt] at (tp) {$t_2$};

    \coordinate (midS0) at ($(s)!0.5!(sp)$);
    \node[mainLbl, above=2pt] at (midS0) {$S_0$};

    \coordinate (midS1) at ($(s)!0.5!(a1)$);
    \node[mainLbl, left=2pt] at (midS1) {$S_1$};

    \coordinate (midS2) at ($(s)!0.5!(a2)$);
    \node[mainLbl, right=2pt] at (midS2) {$S_2$};

    \coordinate (midS3) at ($(sp)!0.5!(a3)$);
    \node[mainLbl, left=2pt] at (midS3) {$S_3$};

    \coordinate (midS4) at ($(sp)!0.5!(a4)$);
    \node[mainLbl, right=2pt] at (midS4) {$S_4$};

    \coordinate (midT1) at ($(t)!0.5!(a1)$);
    \node[greenLbl, left=2pt] at (midT1) {$T_1$};

    \coordinate (midT2) at ($(t)!0.5!(a2)$);
    \node[greenLbl, right=2pt] at (midT2) {$T_2$};

    \coordinate (midT3) at ($(tp)!0.5!(a3)$);
    \node[greenLbl, left=2pt] at (midT3) {$T_3$};

    \coordinate (midT4) at ($(tp)!0.5!(a4)$);
    \node[greenLbl, right=2pt] at (midT4) {$T_4$};

    \coordinate (midT0) at ($(t)!0.5!(tp)$);
    \node[greenLbl, below=2pt] at (midT0) {$T_0$};

    #3
\end{tikzpicture}%
}

\begin{minipage}{\textwidth}
    \centering
    \typeAFrame{}{}{}
\end{minipage}
